An Open and Reconfigurable User Interface to Manage Complex ROS-based Robotic Systems

The Robot Operating System (ROS) has significantly gained popularity among robotic engineers and researchers over the past five years, primarily due to its powerful infrastructure for node communication, which enables developers to build modular and large robotic applications. However, ROS presents a steep learning curve and lacks the intuitive usability of vendor-specific robotic Graphical User Interfaces (GUIs). Moreover, its modular and distributed nature complicates the control and monitoring of extensive systems, even for advanced users. To address these challenges, this paper proposes a highly adaptable and reconfigurable web-based GUI for intuitively controlling, monitoring, and configuring complex ROS-based robotic systems. The GUI leverages ROSBridge and roslibjs to ensure seamless communication with ROS systems via topics and services. Designed as a versatile platform, the GUI allows for the selective incorporation of modular features to accommodate diverse robotic systems and applications. An initial set of commonly used features in robotic applications is presented. To demonstrate its reconfigurability, the GUI was customized and tested for four industrial use cases, receiving positive feedback. The project's repository has been made publicly available to support the robotics community and lower the entry barrier for ROS in industrial applications.

==> Sections/Framework.tex <==
\subsection{Application Framework \textcolor{blue}{P, 0.7 pg}}
\label{sec:framework}



==> Sections/Implementation.tex <==
\section{Implementation}
\label{sec:implementation}

\input{Sections/Use_cases}
\input{Sections/Features}

==> Sections/Overview.tex <==
\subsection{Application Overview \textcolor{blue}{P, 0.7 pg}}
%\subsection{Application overview and common features \textcolor{blue}{P, 0.7 pg}}
\label{sec:overview}

==> Sections/table_reconfiguration_v1.tex <==
\begin{table*}[t]
\renewcommand{\arraystretch}{1.3}
\caption{Reconfiguration of features} \label{tab:reconfig}
\begin{tabular}{l|l}
\hline
\textbf{Feature}                                                                    & \textbf{Reconfigurable parameters}                                                                                                                                                                                                                                                            \\ \hline
Multirole security clearance                                                        & Edit users info in users.json file                                                                                                                                                                                                                                                            \\ \hline
\begin{tabular}[c]{@{}l@{}}Dynamic modules launching \\ and monitoring\end{tabular} & Edit elements of 'launchers' dictionary (name, list of launch files, list of nodes, list of authorized user roles)                                                                                                                                                                            \\ \hline
Sensor data visualization                                                           & Edit elements of 'sensors' dictionary (name, id, graph title, graph type, axes limits, labels, topic, msg type)                                                                                                                                                                               \\ \hline
\begin{tabular}[c]{@{}l@{}}Robot manual motion \\ control\end{tabular}              & \begin{tabular}[c]{@{}l@{}}Edit the list of robot end effectors\\ Edit the list of robot arms\\ Edit the default motion values (speed, acceleration, gripper opening distance)\\ Edit names of topics and services\\ Edit back-end ROS node to interface the specific robot used\end{tabular} \\ \hline
\begin{tabular}[c]{@{}l@{}}Robot automatic motion\\ control\end{tabular}            & \begin{tabular}[c]{@{}l@{}}Edit elements of 'status\_msgs' list (id, displayed name, default value) \\ Edit the names of topics and services \\ Edit back-end ROS node to interface the specific robot used\end{tabular}                                                                      \\ \hline
Video stream visualization                                                          & Edit elements of 'camera\_list' dictionary (id, image topic)                                                                                                                                                                                                                                  \\ \hline
\begin{tabular}[c]{@{}l@{}}System and process \\ configuration\end{tabular}         & \begin{tabular}[c]{@{}l@{}}Edit elements of 'parameters\_msgs' dictionary (param group, displayed name, param id, default value) \\ Edit the parameters list in the config.csv file\end{tabular}                                                                                              \\ \hline
\begin{tabular}[c]{@{}l@{}}Trajectory/routine recording\\ and testing\end{tabular}  & \begin{tabular}[c]{@{}l@{}}Edit the list of motion groups, called 'robot\_groups'\\ Edit the dictionary of robot end effectors, called 'robot\_tools'\\ Edit back-end ROS node to interface the specific robot used\end{tabular}                                                              \\ \hline
Alarms visualization                                                                & Edit the name of the topic that publishes the alarms in 'safety\_topic\_name'                                                                                                                                                                                                                 \\ \hline
Databases update                                                                    & \begin{tabular}[c]{@{}l@{}}Edit the list of files that can be overwritten\\ Edit the path of the database directory\end{tabular}                                                                                                                                                              \\ \hline
\end{tabular}
\end{table*}

==> Sections/test_figures.tex <==
\setlength{\textfloatsep}{8pt}
\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{component_pipeline_2.jpg}
    \caption{UML state machine diagram of the module state transitions. The list of active ROS nodes is checked every second.}
    \label{fig:pipeline2}
\end{figure}

\setlength{\textfloatsep}{8pt}
\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{component_pipeline_3.jpg}
    \caption{UML state machine diagram of the module state transitions. The list of active ROS nodes is checked every second.}
    \label{fig:pipeline3}
\end{figure}
